Krylov-Type Methods for Tensor Computations

Several Krylov-type procedures are introduced that generalize matrix Krylov methods for tensor computations. They are denoted minimal Krylov recursion, maximal Krylov recursion, contracted tensor product Krylov recursion. It is proved that the for a given tensor with low rank, the minimal Krylov recursion extracts the correct subspaces associated to the tensor within certain number of iterations. An optimized minimal Krylov procedure is described that gives a better tensor approximation for a given multilinear rank than the standard minimal recursion. The maximal Krylov recursion naturally admits a Krylov factorization of the tensor. The tensor Krylov methods are intended for the computation of low-rank approximations of large and sparse tensors, but they are also useful for certain dense and structured tensors for computing their higher order singular value decompositions or obtaining starting points for the best low-rank computations of tensors. A set of numerical experiments, using real life and synthetic data sets, illustrate some of the properties of the tensor Krylov methods.

==> myTheorems.tex <==
%%-- This file contais definitions of theorem environments.
%%-- The following needs the amsthm package.

\theoremstyle{plain}% default
\newtheorem{thm}{Theorem}[section]
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem*{cor}{Corollary}

\theoremstyle{definition}
\newtheorem{defn}{Definition}[section]
\newtheorem{conj}{Conjecture}[section]
\newtheorem{exmp}{Example}[section]



\theoremstyle{remark}
\newtheorem{rem}{Remark}[section]
\newtheorem*{note}{Note}
\newtheorem{case}{Case}
\newtheorem{obs}{Observation}[section]

